Understanding (Un)Intended Memorization in Text-to-Image Generative Models

Multimodal machine learning, especially text-to-image models like Stable Diffusion and DALL-E 3, has gained significance for transforming text into detailed images. Despite their growing use and remarkable generative capabilities, there is a pressing need for a detailed examination of these models' behavior, particularly with respect to memorization. Historically, memorization in machine learning has been context-dependent, with diverse definitions emerging from classification tasks to complex models like Large Language Models (LLMs) and Diffusion models. Yet, a definitive concept of memorization that aligns with the intricacies of text-to-image synthesis remains elusive. This understanding is vital as memorization poses privacy risks yet is essential for meeting user expectations, especially when generating representations of underrepresented entities. In this paper, we introduce a specialized definition of memorization tailored to text-to-image models, categorizing it into three distinct types according to user expectations. We closely examine the subtle distinctions between intended and unintended memorization, emphasizing the importance of balancing user privacy with the generative quality of the model outputs. Using the Stable Diffusion model, we offer examples to validate our memorization definitions and clarify their application.

==> sec/orig_results.tex <==
\begin{table*}[h]
\centering
    \begin{tabular}{>{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm}>{\centering\arraybackslash}m{3cm}>{\centering\arraybackslash}m{3cm}>{\centering\arraybackslash}m{2.5cm}>{\centering\arraybackslash}m{2cm}}
    \hline
    \centering \textbf{Memorization\\Types} & \centering \textbf{Input\\Prompt} & \textbf{Generation} & \textbf{Top Match} & \centering \textbf{Matching Prompt} & \textbf{CLIP Similarity Score} \\ \hline 
    \centering \(M_E\) & 
    \centering \small\texttt{High quality image of Elon Musk} & 
    {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/(2x2) high quality image of elon musk.jpg}} & 
    {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/laion_elon.png}} & 
    \centering \small\texttt{Elon Musk} & 
    0.959\\ \hline
    \centering \(M_I\) & 
    \centering \small\texttt{High resolution photo of Istanbul} & 
    {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/(2x2) high resolution photo of Istanbul.jpg}} & 
    {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/laion_istanbul.png}} & 
    \centering \small\texttt{By traveling to these 6 cities, you have seen the whole world!} & 
    0.948 \\ \hline
    \centering \(M_U\) & 
    \centering \small\texttt{When a man came up with a brilliant idea} & 
    {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/(2x2) When a man came up with a brilliant idea.jpg}} & 
    {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/laion_brilliant_idea.png}} & 
    \centering \small\texttt{Miguel Gaspar Almendros Rodríguez} & 
     0.806 \\  
    % \centering \(M_P\) & 
    % \centering \small\texttt{Realistic photo of a boxer fighting in the ring} & 
    % {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/(2x2) realistic photo of a boxer fighting in the ring.jpg}} & 
    % {\includegraphics[width=3cm]{AuthorKit24/AnonymousSubmission/pretrained_images/laion_boxer.png}} & 
    % \centering \small\texttt{Lehigh Valley Kickboxing} & 
    % 0.887 \\
    \hline
    \end{tabular}
    \caption{Images generated using pre-trained Stable Diffusion \cite{rombach2022high} model for different types of memorization and matching (image, prompt) pair from the LAION-5B \cite{schuhmann2022laion} dataset.}
    \label{table:orig_results}
\end{table*}
